DynASP2.5: Dynamic Programming on Tree Decompositions in Action

A vibrant theoretical research area are efficient exact parameterized algorithms. Very recent solving competitions such as the PACE challenge show that there is also increasing practical interest in the parameterized algorithms community. An important research question is whether dedicated parameterized exact algorithms exhibit certain practical relevance and one can even beat well-established problem solvers. We consider the logic-based declarative modeling language and problem solving framework Answer Set Programming (ASP). State-of-the-art ASP solvers rely considerably on Sat-based algorithms. An ASP solver (DynASP2), which is based on a classical dynamic programming on tree decompositions, has been published very recently. Unfortunately, DynASP2 can outperform modern ASP solvers on programs of small treewidth only if the question of interest is to count the number of solutions. In this paper, we describe underlying concepts of our new implementation (DynASP2.5) that shows competitive behavior to state-of-the-art ASP solvers even for finding just one solution when solving problems as the Steiner tree problem that have been modeled in ASP on graphs with low treewidth. Our implementation is based on a novel approach that we call multi-pass dynamic programming (M-DPSINC).

==> commands.tex <==
% Misc
\newcommand{\dneg}{\ensuremath{\operatorname{not}\,}}
\newcommand{\la}{\ensuremath{\leftarrow}}
\newcommand{\HU}[1]{\ensuremath{\mathcal{U}_#1}}
\newcommand{\HB}[1]{\ensuremath{\mathcal{B}_#1}}
\newcommand{\etal}{\emph{{et al}.}\@\xspace}
\newcommand{\eg}{e.g.,\@\xspace}
\newcommand{\ie}{i.e.,\@\xspace}
\newcommand{\wrt}{w.r.t.\@\xspace}
\newcommand{\dflat}{\mbox{D-FLAT}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\problem}[1]{\textsc{#1}}
\newcommand{\predicate}[1]{\texttt{\small #1}}
\newcommand{\dflatItem}[1]{\texttt{#1}}
\newcommand{\I}{\mathcal{I}}
\newcommand\pair[2]{\left< #1,#2 \right>}
\newcommand\tuple[1]{\left< #1 \right>}

\newcommand{\minSat}{\problem{$\subseteq$-Minimal Sat}}
\newcommand{\minDomSet}{\problem{$\subseteq$-Minimal Dominating Set}}
% todo
\newcommand{\todoi}[1]{\todo[inline]{#1}}

% complexity
\newcommand{\complexityclass}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\Sp}[1]{\complexityclass{\Sigma^P_{#1}}}
\newcommand{\Pp}[1]{\complexityclass{\Pi^P_{#1}}}
%\newcommand{\NP}{\complexityclass{NP}}
\newcommand{\coNP}{\complexityclass{\text{co-}NP}}
\newcommand{\DP}{\complexityclass{D^P}}
%\newcommand{\PSPACE}{\mbox{\rm PSPACE}}

% http://tex.stackexchange.com/questions/112204/how-to-vertically-center-the-vdots-in-this-node
\makeatletter
\DeclareRobustCommand{\rvdots}{%
  \vbox{
    \baselineskip4\p@\lineskiplimit\z@
    \kern-\p@
    \hbox{.}\hbox{.}\hbox{.}
  }}
\makeatother

% Algorithms
\newcommand{\eps}{\ensuremath{\operatorname{extensionPointers}}}
\newcommand{\cost}{\ensuremath{\operatorname{cost}}}
\newcommand{\type}{\ensuremath{\operatorname{type}}}
\newcommand{\solCount}{\ensuremath{\operatorname{count}}}


==> graph0/graph_inc.tex <==
\begin{tikzpicture}[node distance=7mm,every node/.style={fill,circle,inner sep=2pt}]
\node (a) [label={[text height=1.5ex,yshift=0.0cm,yshift=-0.15cm]above:$e_{ab}$}] {};
\node (b) [right = 0.5cm of a,label={[text height=1.5ex,yshift=-0.15cm]above:$e_{bc}$}] {};
\node (c) [right = 0.5cm of b,label={[text height=1.5ex,yshift=-0.15cm]above:$e_{cd}$}] {};
\node (d) [right = 0.5cm of c,label={[text height=1.5ex,yshift=-0.15cm]above:$e_{ad}$}] {};
\node (e) [right = 0.5cm of d,label={[text height=1.5ex,yshift=-0.15cm]above:$a_{b}$}] {};
\node (f) [right = 0.5cm of e,label={[text height=1.5ex,yshift=-0.15cm]above:$a_{d}$}] {};
\node (g) [right = 0.5cm of f,label={[text height=1.5ex,yshift=-0.15cm]above:$a_{c}$}] {};
\node (r3) [below = 0.5cm of a,label={[text height=1.5ex,xshift=-0.15cm]right:${r_{ab}}$}] {};
\node (r4) [below = 0.5cm of b,label={[text height=1.5ex,xshift=-0.15cm]right:${r_{bc}}$}] {};
\node (r1) [below = 0.5cm of c,label={[text height=1.5ex,xshift=-0.15cm]right:${r_{cd}}$}] {};
\node (r2) [below = 0.5cm of d,label={[text height=1.5ex,xshift=-0.15cm]right:${r_{ad}}$}] {};
\node (r5) [right = 0.5cm of r2,label={[text height=1.5ex,xshift=-0.15cm]right:${r_{b}}$}] {};
\node (r6) [right = 0.5cm of r5,label={[text height=1.5ex,xshift=-0.15cm]right:${r_{d}}$}] {};
\node (r7) [right = 0.5cm of r6,label={[text height=1.5ex,xshift=-0.15cm]right:${r_{c1}}$}] {};
\node (r8) [right = 0.5cm of r7,label={[text height=1.5ex,xshift=-0.15cm]right:${r_{c2}}$}] {};
\node (r9) [right = 0.5cm of r8,label={[text height=1.5ex,xshift=-0.15cm]right:${r_{\neg c}}$}] {};
%\node (e) [right of = d,label={[text height=1.5ex]above:$e$}] {};
\draw (a) to (r3);
\draw (e) to (r3);

\draw (b) to (r4);
\draw (e) to (r4);
%\draw (a) to (c);
\draw (c) to (r1);
\draw (f) to (r1);

\draw (d) to (r2);
\draw (f) to (r2);

\draw (a) to (r5);
\draw (e) to (r5);

\draw (d) to (r6);
\draw (f) to (r6);

\draw (g) to (r9);

\draw (g) to (r8);
\draw (d) to (r8);
\draw (f) to (r8);


\draw (g) to (r7);
\draw (b) to (r7);
\draw (e) to (r7);



\end{tikzpicture}


==> graph0/graph_inp.tex <==
\begin{tikzpicture}[node distance=7mm,every node/.style={fill,circle,inner sep=2pt}]
\node (a) [fill=red,label={[text height=1.5ex,yshift=0.0cm,yshift=-0.1cm]above:$a$}] {};
\node (b) [draw,right = 0.5cm of a,yshift=-0.5cm,label={[text height=1.5ex,yshift=-0.1cm]above:$b$}] {};
\node (c) [fill=red,right = 0.5cm of b,yshift=0.5cm,label={[text height=1.5ex,yshift=-0.1cm]above:$c$}] {};
\node (d) [draw,above = 0.75cm of b,label={[text height=1.5ex,yshift=-0.1cm]above:$d$}] {};
\draw (a) to (b);
\draw (b) to (c);
\draw (d) to (c);
\draw (a) to (d);

\end{tikzpicture}


==> graph0/td_inc.tex <==
\begin{tikzpicture}[node distance=0.5mm]
%\tikzset{every node/.style=tdnode}
\tikzset{every path/.style=thick}

\node (leaf0) [tdnode,label={[]left:$t_1$}] {$\{b, c, {r_1}, {r_2}\}$};
\node (leaf1) [tdnode,label={[xshift=0em]left:$t_2$}, above = 0.1cm of leaf0] {$\{a,b,{r_1}, {r_2}\}$};
\node (leaf2) [tdnode,label={[xshift=0em,yshift=-0.2em]above right:$t_3$}, right = 0.1cm of leaf0]  {$\{a, d, {r_3}\}$};
\coordinate (middle) at ($ (leaf1.north east)!.5!(leaf2.north west) $);
\node (join) [tdnode,ultra thick,label={[xshift=-0.25em,yshift=0.4em]right:$t_4$}, right = 0.15cm of leaf1] {$\{a\}$}; %above  = 1mm of middle

\draw [->] (leaf0) to (leaf1);
\draw [<-] (join) to (leaf1);
\draw [<-] (join) to (leaf2);
\end{tikzpicture}


==> graph0/td_inc2.tex <==
\begin{tikzpicture}[node distance=0.5mm]
%\tikzset{every node/.style=tdnode}
\tikzset{every path/.style=thick}

\node (leaf0) [tdnode,label={[xshift=0.12cm]left:$t_1$}] {$\{r_{ab}, e_{ab}\}$};
\node (leaf1) [tdnode,label={[xshift=0.12cm]left:$t_2$}, above = 0.1cm of leaf0] {$\{r_b, e_{ab}, a_b\}$};
\node (exch1) [tdnode,label={[xshift=-0.12cm]right:$t_3$}, right = 0.2cm of leaf1] {$\{r_{bc}, e_{bc}, a_b\}$};
\node (exch2) [tdnode,label={[xshift=0.12cm]left:$t_4$}, below = 0.1cm of exch1, xshift=0.1cm] {$\{r_{c1}, e_{bc}, a_b\}$};
\node (exch25) [tdnode,label={[xshift=-0.12cm]right:$t_5$}, right = 0.2cm of exch2] {$\{r_{c1}, a_c\}$};
%\coordinate (middle) at ($ (leaf1.north east)!.5!(leaf2.north west) $);
\node (join) [tdnode,ultra thick,label={[xshift=0.12cm]left:$t_{11}$}, right = 0.75cm of exch1] {$\{r_{\neg c}, a_c\}$}; %above  = 1mm of middle
\node (exch4) [tdnode,label={[xshift=0.12cm]left:$t_8$}, right = 0.4cm of join]  {$\{r_{cd}, e_{cd}, a_d\}$};
\node (interr) [tdnode,label={[xshift=0.12cm,yshift=-0.1cm]left:$t_{10}$}, below = 0.1cm of exch4, xshift=-0.5cm] {$\{r_{c2}, a_c\}$}; %above  = 1mm of middle
\node (interr2) [tdnode,label={[xshift=-0.12cm]right:$t_9$}, right = 0.2cm of interr] {$\{r_{c2}, e_{cd}, a_d\}$}; %above  = 1mm of middle
\node (leaf2) [tdnode,label={[xshift=-0.12cm]right:$t_7$}, right = 0.2cm of exch4]  {$\{r_d, e_{ad}, a_d\}$};
\node (exch3) [tdnode,label={[xshift=-0.12cm]right:$t_6$}, below = 0.1cm of leaf2, xshift=1.4cm]  {$\{r_{ad}, e_{ad}\}$};

\draw [->] (leaf0) to (leaf1);
\draw [->] (exch3) to (leaf2);
\draw [<-] (exch1) to (leaf1);
\draw [<-] (exch2) to (exch1);
\draw [<-] (exch25) to (exch2);
\draw [->] (exch25) to (join);
\draw [->] (leaf2) to (exch4);
\draw [<-] (interr2) to (exch4);
\draw [<-] (interr) to (interr2);
\draw [->] (interr.west) to (join);
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: ipec2017
%%% End:

==> graph0_norm/tables/join.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle \tuplecolor{\inputPredColor}{M_{11.i}} \rangle$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\langle \tuplecolor{\inputPredColor}{\emptyset} \rangle$ \\\hline
$\langle \tuplecolor{\inputPredColor}{\{a\}} \rangle$\\
\end{tabular}


==> graph0_norm/tables/join_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle \tuplecolor{\inputPredColor}{M_{11.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{11.i}} \rangle$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle $\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\outputPredColor}{\{\{a\}\}} \rangle $\\
\end{tabular}


==> graph0_norm/tables/join_aspnum.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$i$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$1$\\\hline
$2$\\\hline
$3$\\
\end{tabular}


==> graph0_norm/tables/join_aspnumb.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$j$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
\\\hline
\\\hline
$1$\\
\end{tabular}


==> graph0_norm/tables/joinnum.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$1$ \\\hline
$2$\\
\end{tabular}


==> graph0_norm/tables/leaf0.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\langle \tuplecolor{\inputPredColor}{M_{4.i}} \rangle$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\langle \tuplecolor{\inputPredColor}{\{c\}}\rangle$\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a\}}\rangle$\\\hline
$\langle\tuplecolor{\inputPredColor}{\{a,c\}}\rangle$\\\hline
$\langle\tuplecolor{\inputPredColor}{\{b,c\}}\rangle$\\\hline
$\langle\tuplecolor{\inputPredColor}{\{a,b,c\}}\rangle$\\
\end{tabular}


==> graph0_norm/tables/leaf00.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\langle \tuplecolor{\inputPredColor}{M_{1.i}} \rangle$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\langle \tuplecolor{\inputPredColor}{\emptyset}\rangle$
\end{tabular}


==> graph0_norm/tables/leaf00_asp.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\langle \tuplecolor{\inputPredColor}{M_{1.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{1.i}}  \rangle$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\emptyset}\rangle$
\end{tabular}


==> graph0_norm/tables/leaf00_aspnum.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\ % & \multicolumn{1}{c}{$M_i$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$1$
\end{tabular}


==> graph0_norm/tables/leaf00_aspnumb.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$j$}\\ % & \multicolumn{1}{c}{$M_i$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$1$
\end{tabular}


==> graph0_norm/tables/leaf00num.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\ % & \multicolumn{1}{c}{$M_i$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$1$
\end{tabular}


==> graph0_norm/tables/leaf0_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle \tuplecolor{\inputPredColor}{M_{4.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{4.i}} \rangle $}\\
\hline\hline
$\langle \tuplecolor{\inputPredColor}{\{c\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle $\\\hline
%$1.1$ & & & T\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle $\\\hline
%$1.2$ & T & &\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a,c\}}, \tuplecolor{\outputPredColor}{\{\{a\}\}} \rangle $\\\hline
%$1.3$ & T & & T & $1.3.1$ & T&\\\hline
$\langle \tuplecolor{\inputPredColor}{\{b,c\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle $\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a,b,c\}}, \tuplecolor{\outputPredColor}{\{\{a\}\}} \rangle $\\
%$1.4$ & & T & T\\\hline
%$1.5$ & T & T & T & $1.5.1$ & T&\\
\end{tabular}


==> graph0_norm/tables/leaf0_aspnum.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\
\hline\hline
$1$\\\hline
$2$\\\hline
$3$\\\hline
$4$\\\hline
$5$
\end{tabular}



==> graph0_norm/tables/leaf0_aspnumb.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$j$}\\
\hline\hline
\\\hline
\\\hline
$1$\\\hline
\\\hline
$1$\\
\end{tabular}


==> graph0_norm/tables/leaf0num.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\ % & \multicolumn{1}{c}{$M_i$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$1$ \\\hline
$2$ \\\hline
$3$ \\\hline
$4$ \\\hline
$5$ \\
\end{tabular}


==> graph0_norm/tables/leaf1.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle \tuplecolor{\inputPredColor}{M_{9.i}} \rangle$}\\ % & \multicolumn{2}{c}{$M_i$}\\
%& $a$ & $d$ \\
\hline\hline
$\langle \tuplecolor{\inputPredColor}{\{a\}}\rangle$\\\hline
$\langle \tuplecolor{\inputPredColor}{\{d\}}\rangle$\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a,d\}}\rangle$\\
\end{tabular}


==> graph0_norm/tables/leaf1_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle \tuplecolor{\inputPredColor}{M_{9.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{9.i}} \rangle $}\\
\hline\hline
$\langle \tuplecolor{\inputPredColor}{\{ a\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\\hline
$\langle \tuplecolor{\inputPredColor}{\{d\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle $\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a,d\}}, \tuplecolor{\outputPredColor}{\{\{a\},} $\\
$\qquad\qquad \tuplecolor{\outputPredColor}{\{d\}\}}\rangle$\\
\end{tabular}


==> graph0_norm/tables/leaf1_aspnum.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\
\hline\hline
$1$\\\hline
$2$\\\hline
\multirow{2}{*}{$3$}\\
\end{tabular}


==> graph0_norm/tables/leaf1_aspnumb.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$j$}\\
\hline\hline
\\\hline
\\\hline
$1$\\
$2$\\
\end{tabular}


==> graph0_norm/tables/leaf1num.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\ % & \multicolumn{2}{c}{$M_i$}\\
%& $a$ & $d$ \\
\hline\hline
$1$\\\hline
$2$\\\hline
$3$\\
\end{tabular}


==> graph0_norm/tables_inc/join.tex <==
\begin{tabular}{l}
\multirow{1}{*}{\pcrop$\langle \tuplecolor{\inputPredColor}{M_{6.i}}, \tuplecolor{\statePredColor}{\sigma_{6.i}} \rangle\quad\;\;\tab{6}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{b\}}, \tuplecolor{\statePredColor}{\{r_2\}} \rangle\pcrop$ \\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{b\}}, \tuplecolor{\statePredColor}{\{r_1\}} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}} \rangle$\\
\end{tabular}


==> graph0_norm/tables_inc/join_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{6.i}}, \tuplecolor{\statePredColor}{\sigma_{6.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{6.i}} \rangle\quad\;\tab{6}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{c\}}, \tuplecolor{\statePredColor}{\{r_1\mapstos0,r_2\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\{}$\\
$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\})\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{c\}}, \tuplecolor{\statePredColor}{\{r_1\mapstos0,r_2\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\{}$\\
$\quad\tuplecolor{\outputPredColor}{(\{c\}, \{r_1\mapstos1, r_2\mapstos\infty\}),}\pcrop$\\
$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\}),}$\\
$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos1\})\}}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty,r_2\mapstos0\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty,r_2\mapstos1\}}, \tuplecolor{\outputPredColor}{\{}$\\
$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\})\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph0_norm/tables_inc/leaf0.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{4.i}}, \tuplecolor{\statePredColor}{\sigma_{4.i}} \rangle \quad\;\;\tab{4}\pcrop$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{c\}}, \tuplecolor{\statePredColor}{\{r_2\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}\rangle$\\
\end{tabular}


==> graph0_norm/tables_inc/leaf00.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{1.i}}, \tuplecolor{\statePredColor}{\sigma_{1.i}} \rangle\;\;\tab{1}\pcrop$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\emptyfunc}\rangle$
\end{tabular}


==> graph0_norm/tables_inc/leaf00_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\tuplecolor{\outputPredColor}{\langle C_{1.i}, \rho_{1.i} \rangle}\quad\qquad\;\tab{1}^{\INCCOUNTERSAT}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\hspace{-0.85em}\tuplecolor{\outputPredColor}{\langle\{a_1,f\}, \{r_{cf}\}\rangle, \langle\{a_2, f\}, \{r_{cf}\}\rangle,}\pcrop$\\%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
$\hspace{-0.85em}\tuplecolor{\outputPredColor}{\langle\{f\}, \{r_{cf}\}\rangle, \langle\{a_1,a_2\}, \{r_c\}\rangle, \langle\{}\pcrop$\\%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
$\hspace{-0.85em}\tuplecolor{\outputPredColor}{a_1\}, \{r_c\}\rangle, \langle\{a_2\}, \{r_c\}\rangle, \langle\emptyset, \{r_c\}\rangle}\pcrop\hspace{-0.15em}$\\%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
%$\;\tuplecolor{\outputPredColor}{\langle\{a_1\}, \{r_c\}\rangle, }$%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
%$\;\tuplecolor{\outputPredColor}{\langle\emptyset, \{r_1\}\rangle\}}\rangle\pcrop$\\\hline
%$\quad\tuplecolor{\outputPredColor}{\langle\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\}\rangle,}$\\
%$\quad\tuplecolor{\outputPredColor}{\langle\emptyset, \{r_1\mapstos\infty, r_2\mapstos1\}\rangle\}}\rangle\pcrop$\\\hline
%
%$\;\tuplecolor{\outputPredColor}{\langle\{a\},\{r_1\}\rangle\}}\rangle$\\\hline
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{\langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph0_norm/tables_inc/leaf0_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{4.i}}, \tuplecolor{\statePredColor}{\sigma_{4.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{4.i}} \rangle\quad\tab{4}\pcrop$}\\
\hline\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{c\}}, \tuplecolor{\statePredColor}{\{r_1\mapstos0,r_2\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\{}$\\
$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\})\}}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty,r_2\mapstos0\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$
\end{tabular}


==> graph0_norm/tables_inc/leaf1.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{15.i}}, \tuplecolor{\statePredColor}{\sigma_{15.i}} \rangle\pcrop$}\\ % & \multicolumn{2}{c}{$M_i$}\\
%& $a$ & $d$ \\
\hline\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a,d\}}, \tuplecolor{\statePredColor}{\emptyfunc}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\statePredColor}{\emptyfunc}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{d\}}, \tuplecolor{\statePredColor}{\emptyfunc}\rangle$\\
\end{tabular}


==> graph0_norm/tables_inc/leaf1_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{15.i}}, \tuplecolor{\statePredColor}{\sigma_{15.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{15.i}} \rangle\;\;\tab{15}\pcrop$}\\
\hline\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a,d\}}, \tuplecolor{\statePredColor}{\emptyfunc}, \tuplecolor{\outputPredColor}{\{}$%\\
$\tuplecolor{\outputPredColor}{(\{a\}, \emptyfunc),}\pcrop$\\
$\;\tuplecolor{\outputPredColor}{(\{d\}, \emptyfunc)\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a\}},  \tuplecolor{\statePredColor}{\emptyfunc}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{d\}}, \tuplecolor{\statePredColor}{\emptyfunc}, \tuplecolor{\outputPredColor}{\emptyset} \rangle $
\end{tabular}


==> graph0_norm/tables_inc/r14.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{9.i}}, \tuplecolor{\statePredColor}{\sigma_{9.i}} \rangle\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\statePredColor}{\{r_1\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}} \rangle$\\%\hline
%$\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty,r_2\mapstos1\}} \rangle$\\
\end{tabular}


==> graph0_norm/tables_inc/r14_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{9.i}}, \tuplecolor{\statePredColor}{\sigma_{9.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{9.i}} \rangle\,\;\;\qquad\tab{9}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{(\{a\},\{r_1\}),}\pcrop$\\%\rangle$\\\hline
$\;\tuplecolor{\outputPredColor}{(\emptyset, \emptyset)\}}\rangle$\\\hline
%
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{(\{a\},\{r_1\})\}}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\emptyset}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{(\emptyset,\emptyset)\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\emptyset}\rangle$\\%\hline
%$\tuplecolor{\outputPredColor}{(\emptyset,\hspace{-0.2em}\{r_1\mapstos0\}),}\pcrop$\\
%$\quad\tuplecolor{\outputPredColor}{(\{a\}, \{r_1\mapstos\infty\})\}}\rangle$\\\hline
%
%$\pcrop\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\{}$\\
%$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos0\}),}$%\\
%$\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos1\}),}\pcrop$\\
%$\quad\tuplecolor{\outputPredColor}{(\{a\}, \{r_1\mapstos\infty\}),}$\\
%$\quad\tuplecolor{\outputPredColor}{(\{a\}, \{r_1\mapstos1\})\}}\rangle$\\\hline
%
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\emptyset}\rangle$\\\hline
%
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos1\})\}}\rangle\pcrop$\\
\end{tabular}


==> graph0_norm/tables_inc/r5.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{5.i}}, \tuplecolor{\statePredColor}{\sigma_{5.i}} \rangle \;\tab{5}\pcrop$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{b,c\}}, \tuplecolor{\statePredColor}{\{r_2\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{b\}}, \tuplecolor{\statePredColor}{\{r_1\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{c\}}, \tuplecolor{\statePredColor}{\{r_2\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}\rangle$\\
\end{tabular}


==> graph0_norm/tables_inc/r5_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{3.i}}, \tuplecolor{\statePredColor}{\sigma_{3.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{3.i}} \rangle\quad\;\tab{3}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$3$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,a_2,f\}}, \tuplecolor{\statePredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\emptyset}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_2,f\}}, \tuplecolor{\statePredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph0_norm/tables_inc/r5_asp_2mdp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{3.i}}, \tuplecolor{\statePredColor}{\sigma_{3.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{3.i}} \rangle\quad\qquad\;\tab{3}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$3$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,a_2,f\}}, \tuplecolor{\statePredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\emptyset}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_2,f\}}, \tuplecolor{\statePredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph0_norm/tables_inc/r7.tex <==
\begin{tabular}{l}
\multirow{1}{*}{\pcrop$\langle \tuplecolor{\inputPredColor}{M_{7.i}}, \tuplecolor{\statePredColor}{\sigma_{7.i}} \rangle\quad\;\;\tab{7}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a,b\}}, \tuplecolor{\statePredColor}{\{r_1,r_2\}} \rangle\pcrop$ \\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a,b\}}, \tuplecolor{\statePredColor}{\{r_1\}} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1,r_2\}} \rangle$
\end{tabular}


==> graph0_norm/tables_inc/r8.tex <==
\begin{tabular}{l}
\multirow{1}{*}{\pcrop$\langle \tuplecolor{\inputPredColor}{M_{8.i}}, \tuplecolor{\statePredColor}{\sigma_{8.i}} \rangle\tab{8}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a,b\}}, \tuplecolor{\statePredColor}{\{r_1\}} \rangle\pcrop$ \\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\statePredColor}{\{r_1\}} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{b\}}, \tuplecolor{\statePredColor}{\{r_1\}} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}} \rangle$
\end{tabular}


==> graph0_norm/tables_inc/r8_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{8.i}}, \tuplecolor{\statePredColor}{\sigma_{8.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{8.i}} \rangle\quad\qquad\;\tab{8}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a,b\}}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{(\{a\}, \{r_1\}),}\pcrop$\\
$\;\tuplecolor{\outputPredColor}{(\emptyset, \emptyset)\}}\rangle$\\\hline%b\}, \{r_1\}), (\emptyset, \{r_1\})\}} \rangle\pcrop$\\\hline
%$\;\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}}\rangle\pcrop$\\\hline
%$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\}),}$\\
%$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos1\})\}}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{(\{a\}, \{r_1\})\}}\rangle\pcrop$\\\hline
%$\;\tuplecolor{\outputPredColor}{(\{a\},\{r_1\})\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{b\}}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{(\emptyset,\emptyset)\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$%\\\hline
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph0_norm/tables_inc/r8_asp_2.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{1.i}}, \tuplecolor{\statePredColor}{\sigma_{1.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{1.i}} \rangle\quad\qquad\qquad\qquad\;\tab{1}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,a_2,f\}}, \tuplecolor{\statePredColor}{\{r_c, r_{cf}\}}, \tuplecolor{\outputPredColor}{\{}\pcrop$\\
$\hspace{-0.35em}\tuplecolor{\outputPredColor}{\langle\{a_1,f\}, \{r_{cf}\}\rangle, \langle\{a_2, f\}, \{r_{cf}\}\rangle,}$\\%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
$\hspace{-0.35em}\tuplecolor{\outputPredColor}{\langle\{f\}, \{r_{cf}\}\rangle, \langle\{a_1,a_2\}, \{r_c\}\rangle, }$\\%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
$\hspace{-0.35em}\tuplecolor{\outputPredColor}{\langle\{a_1\}, \{r_c\}\rangle, \langle\{a_2\}, \{r_c\}\rangle, \langle\emptyset, \{r_c\}\rangle\}}\rangle\pcrop$\\\hline%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
%$\;\tuplecolor{\outputPredColor}{}\rangle$\\%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
%$\;\tuplecolor{\outputPredColor}{\langle\emptyset, \{r_1\}\rangle\}}\rangle\pcrop$\\\hline
%$\quad\tuplecolor{\outputPredColor}{\langle\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\}\rangle,}$\\
%$\quad\tuplecolor{\outputPredColor}{\langle\emptyset, \{r_1\mapstos\infty, r_2\mapstos1\}\rangle\}}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,a_2\}}, \tuplecolor{\statePredColor}{\{r_c, r_{cf}\}}, \tuplecolor{\outputPredColor}{\{\langle\{a_1\}, \{r_c, r_{cf}\}\rangle,}\pcrop$\\
$\hspace{-0.35em}\tuplecolor{\outputPredColor}{ \langle\{a_2\}, \{r_c, r_{cf}\}\rangle, \langle\emptyset, \{r_c, r_{cf}\}\rangle\}}\rangle$\\\hline%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
%
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,f\}}, \tuplecolor{\statePredColor}{\{r_c, r_{cf}\}}, \tuplecolor{\outputPredColor}{\{\langle\{f\}, \{r_{cf}\}\rangle,}\pcrop$\\
$\hspace{-0.35em}\tuplecolor{\outputPredColor}{\langle\{a_1\}, \{r_{c}\}\rangle, \langle\emptyset, \{r_c\}\rangle\}}\rangle$\\\hline%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1\}}, \tuplecolor{\statePredColor}{\{r_c, r_{cf}\}}, \tuplecolor{\outputPredColor}{\{\langle\emptyset, \{r_c, r_f\}\rangle\}}\rangle$\\\hline
%$\;\tuplecolor{\outputPredColor}{\langle\{a\},\{r_1\}\rangle\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_2,f\}}, \tuplecolor{\statePredColor}{\{r_c,r_{cf}\}}, \tuplecolor{\outputPredColor}{\{\langle\{a_2\}, \{r_c\}\rangle,}\pcrop$\\
$\hspace{-0.35em}\tuplecolor{\outputPredColor}{ \langle\{f\}, \{r_{cf}\}\rangle \}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_2\}}, \tuplecolor{\statePredColor}{\{r_c, r_{cf}\}}, \tuplecolor{\outputPredColor}{\{\langle\emptyset,\{r_c, r_{cf}\}\rangle\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{f\}}, \tuplecolor{\statePredColor}{\{r_c, r_{cf}\}}, \tuplecolor{\outputPredColor}{\{\langle\emptyset, \{r_c\}\rangle\}} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_c, r_{cf}\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{\langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph0_norm/tables_inc/r8_asp_2mdp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{1.i}}, \tuplecolor{\statePredColor}{\sigma_{1.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{1.i}} \rangle\quad\qquad\;\tab{1}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,a_2,f\}}, \tuplecolor{\statePredColor}{\{r_c, r_{cf}\}}, \tuplecolor{\outputPredColor}{\emptyset}\pcrop$\\
%$\;\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}}\rangle\pcrop$\\\hline
%$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\}),}$\\
%$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos1\})\}}\rangle\pcrop$\\\hline
%
%$\;\tuplecolor{\outputPredColor}{(\{a\},\{r_1\})\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_2,f\}}, \tuplecolor{\statePredColor}{\{r_c,r_{cf}\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph0_norm/tables_inc/r8_asp_2mdp_tmp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{1.i}}, \tuplecolor{\statePredColor}{\sigma_{1.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{1.i}} \rangle\quad\qquad\;\tab{1}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,a_2,f\}}, \tuplecolor{\statePredColor}{\{r_c, r_{cf}\}}, \tuplecolor{\outputPredColor}{}\pcrop$\\
$\;\tuplecolor{\outputPredColor}{(\{a_1,f\}, \{r_{cf}\}), (\{a_2, f\}, \{r_{cf}\}),}$\\%b\}, \{r_1\}), (\emptyset, \{r_1\})\}} \rangle\pcrop$\\\hline
$\;\tuplecolor{\outputPredColor}{(\{f\}, \{r_{cf}\}),}$\\%b\}, \{r_1\}), (\emptyset, \{r_1\})\}} \rangle\pcrop$\\\hline
$\;\tuplecolor{\outputPredColor}{(\{a_1,a_2\}, \{r_c\}), (\{a_1\}, \{r_c\})\}}\rangle$\\%b\}, \{r_1\}), (\emptyset, \{r_1\})\}} \rangle\pcrop$\\\hline
$\;\tuplecolor{\outputPredColor}{(\{a_2\}, \{r_c\}), (\{a_1\}, \{r_c\}), (\emptyset, \{r_c\})\}}\rangle$\\\hline%b\}, \{r_1\}), (\emptyset, \{r_1\})\}} \rangle\pcrop$\\\hline
%$\;\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}}\rangle\pcrop$\\\hline
%$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\}),}$\\
%$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos1\})\}}\rangle\pcrop$\\\hline
%
%$\;\tuplecolor{\outputPredColor}{(\{a\},\{r_1\})\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_2,f\}}, \tuplecolor{\statePredColor}{\{r_c,r_{cf}\}}, \tuplecolor{\outputPredColor}{\{(\{a_2\}, \{r_c\}), (\{f\}, \{r_{cf}\}) \}} \rangle$\\
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph0_norm/tables_inc/r9_asp_2.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{2.i}}, \tuplecolor{\statePredColor}{\sigma_{2.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{2.i}} \rangle\quad\;\tab{2}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,a_2,f\}}, \tuplecolor{\statePredColor}{\{r_f, r_2\}}, \tuplecolor{\outputPredColor}{\emptyset}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,a_2\}}, \tuplecolor{\statePredColor}{\{r_2\}}, \tuplecolor{\outputPredColor}{\{}\pcrop$\\
$\tuplecolor{\outputPredColor}{\hspace{-0.4em}\langle\{a_1\},\emptyset\rangle,}\pcrop$\\%b\}, \{r_1\}), (\emptyset, \{r_1\})\}} \rangle\pcrop$\\\hline
$\tuplecolor{\outputPredColor}{\hspace{-0.4em}\langle\{a_2\}, \{r_2\}\rangle, \langle\emptyset, \emptyset\rangle\}}\rangle\pcrop$\\\hline%b\}, \{r_1\}), (\emptyset, \{r_1\})\}} \rangle\pcrop$\\\hline
%
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,f\}}, \tuplecolor{\statePredColor}{\{r_{f}\}}, \tuplecolor{\outputPredColor}{\emptyset}\rangle$\\\hline
%$\;\tuplecolor{\outputPredColor}{\emptyset}\rangle$\\\hline%b\}, \{r_1\}), (\emptyset, \{r_1\})\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1\}}, \tuplecolor{\statePredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\{\langle\emptyset, \emptyset\rangle\}}\rangle$\\\hline
%$\;\tuplecolor{\outputPredColor}{(\{a\},\{r_1\})\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_2,f\}}, \tuplecolor{\statePredColor}{\{r_{f}, r_2\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_2\}}, \tuplecolor{\statePredColor}{\{r_2\}}, \tuplecolor{\outputPredColor}{\{\langle\emptyset,\emptyset\rangle\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{f\}}, \tuplecolor{\statePredColor}{\{r_f\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$%\\\hline
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph0_norm/tables_inc/r9_asp_2mdp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{2.i}}, \tuplecolor{\statePredColor}{\sigma_{2.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{2.i}} \rangle\quad\qquad\;\tab{2}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,a_2,f\}}, \tuplecolor{\statePredColor}{\{r_f, r_2\}}, \tuplecolor{\outputPredColor}{\emptyset}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_2,f\}}, \tuplecolor{\statePredColor}{\{r_{f}, r_2\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph1_norm/tables/join.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle \tuplecolor{\inputPredColor}{M_{11.i}} \rangle$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\langle \tuplecolor{\inputPredColor}{\emptyset} \rangle$ \\\hline
$\langle \tuplecolor{\inputPredColor}{\{a\}} \rangle$\\
\end{tabular}


==> graph1_norm/tables/join_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle \tuplecolor{\inputPredColor}{M_{11.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{11.i}} \rangle$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle $\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\outputPredColor}{\{\{a\}\}} \rangle $\\
\end{tabular}


==> graph1_norm/tables/join_aspnum.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$i$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$1$\\\hline
$2$\\\hline
$3$\\
\end{tabular}


==> graph1_norm/tables/join_aspnumb.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$j$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
\\\hline
\\\hline
$1$\\
\end{tabular}


==> graph1_norm/tables/joinnum.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$1$ \\\hline
$2$\\
\end{tabular}


==> graph1_norm/tables/leaf0.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\langle \tuplecolor{\inputPredColor}{M_{4.i}} \rangle$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\langle \tuplecolor{\inputPredColor}{\{c\}}\rangle$\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a\}}\rangle$\\\hline
$\langle\tuplecolor{\inputPredColor}{\{a,c\}}\rangle$\\\hline
$\langle\tuplecolor{\inputPredColor}{\{b,c\}}\rangle$\\\hline
$\langle\tuplecolor{\inputPredColor}{\{a,b,c\}}\rangle$\\
\end{tabular}


==> graph1_norm/tables/leaf00.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\langle \tuplecolor{\inputPredColor}{M_{1.i}} \rangle$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\langle \tuplecolor{\inputPredColor}{\emptyset}\rangle$
\end{tabular}


==> graph1_norm/tables/leaf00_asp.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\langle \tuplecolor{\inputPredColor}{M_{1.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{1.i}}  \rangle$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\emptyset}\rangle$
\end{tabular}


==> graph1_norm/tables/leaf00_aspnum.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\ % & \multicolumn{1}{c}{$M_i$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$1$
\end{tabular}


==> graph1_norm/tables/leaf00_aspnumb.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$j$}\\ % & \multicolumn{1}{c}{$M_i$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$1$
\end{tabular}


==> graph1_norm/tables/leaf00num.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\ % & \multicolumn{1}{c}{$M_i$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$1$
\end{tabular}


==> graph1_norm/tables/leaf0_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle \tuplecolor{\inputPredColor}{M_{4.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{4.i}} \rangle $}\\
\hline\hline
$\langle \tuplecolor{\inputPredColor}{\{c\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle $\\\hline
%$1.1$ & & & T\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle $\\\hline
%$1.2$ & T & &\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a,c\}}, \tuplecolor{\outputPredColor}{\{\{a\}\}} \rangle $\\\hline
%$1.3$ & T & & T & $1.3.1$ & T&\\\hline
$\langle \tuplecolor{\inputPredColor}{\{b,c\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle $\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a,b,c\}}, \tuplecolor{\outputPredColor}{\{\{a\}\}} \rangle $\\
%$1.4$ & & T & T\\\hline
%$1.5$ & T & T & T & $1.5.1$ & T&\\
\end{tabular}


==> graph1_norm/tables/leaf0_aspnum.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\
\hline\hline
$1$\\\hline
$2$\\\hline
$3$\\\hline
$4$\\\hline
$5$
\end{tabular}



==> graph1_norm/tables/leaf0_aspnumb.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$j$}\\
\hline\hline
\\\hline
\\\hline
$1$\\\hline
\\\hline
$1$\\
\end{tabular}


==> graph1_norm/tables/leaf0num.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\ % & \multicolumn{1}{c}{$M_i$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$1$ \\\hline
$2$ \\\hline
$3$ \\\hline
$4$ \\\hline
$5$ \\
\end{tabular}


==> graph1_norm/tables/leaf1.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle \tuplecolor{\inputPredColor}{M_{9.i}} \rangle$}\\ % & \multicolumn{2}{c}{$M_i$}\\
%& $a$ & $d$ \\
\hline\hline
$\langle \tuplecolor{\inputPredColor}{\{a\}}\rangle$\\\hline
$\langle \tuplecolor{\inputPredColor}{\{d\}}\rangle$\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a,d\}}\rangle$\\
\end{tabular}


==> graph1_norm/tables/leaf1_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle \tuplecolor{\inputPredColor}{M_{9.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{9.i}} \rangle $}\\
\hline\hline
$\langle \tuplecolor{\inputPredColor}{\{ a\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\\hline
$\langle \tuplecolor{\inputPredColor}{\{d\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle $\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a,d\}}, \tuplecolor{\outputPredColor}{\{\{a\},} $\\
$\qquad\qquad \tuplecolor{\outputPredColor}{\{d\}\}}\rangle$\\
\end{tabular}


==> graph1_norm/tables/leaf1_aspnum.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\
\hline\hline
$1$\\\hline
$2$\\\hline
\multirow{2}{*}{$3$}\\
\end{tabular}


==> graph1_norm/tables/leaf1_aspnumb.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$j$}\\
\hline\hline
\\\hline
\\\hline
$1$\\
$2$\\
\end{tabular}


==> graph1_norm/tables/leaf1num.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\ % & \multicolumn{2}{c}{$M_i$}\\
%& $a$ & $d$ \\
\hline\hline
$1$\\\hline
$2$\\\hline
$3$\\
\end{tabular}


==> graph1_norm/tables_inc/join.tex <==
\begin{tabular}{l}
\multirow{1}{*}{\pcrop$\langle \tuplecolor{\inputPredColor}{M_{6.i}}, \tuplecolor{\statePredColor}{\sigma_{6.i}} \rangle\quad\;\;\tab{6}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{b\}}, \tuplecolor{\statePredColor}{\{r_2\}} \rangle\pcrop$ \\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{b\}}, \tuplecolor{\statePredColor}{\{r_1\}} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}} \rangle$\\
\end{tabular}


==> graph1_norm/tables_inc/join_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{6.i}}, \tuplecolor{\statePredColor}{\sigma_{6.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{6.i}} \rangle\quad\;\tab{6}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{c\}}, \tuplecolor{\statePredColor}{\{r_1\mapstos0,r_2\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\{}$\\
$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\})\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{c\}}, \tuplecolor{\statePredColor}{\{r_1\mapstos0,r_2\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\{}$\\
$\quad\tuplecolor{\outputPredColor}{(\{c\}, \{r_1\mapstos1, r_2\mapstos\infty\}),}\pcrop$\\
$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\}),}$\\
$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos1\})\}}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty,r_2\mapstos0\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty,r_2\mapstos1\}}, \tuplecolor{\outputPredColor}{\{}$\\
$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\})\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph1_norm/tables_inc/leaf0.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{4.i}}, \tuplecolor{\statePredColor}{\sigma_{4.i}} \rangle \quad\;\;\tab{4}\pcrop$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{c\}}, \tuplecolor{\statePredColor}{\{r_2\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}\rangle$\\
\end{tabular}


==> graph1_norm/tables_inc/leaf00.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{1.i}}, \tuplecolor{\statePredColor}{\sigma_{1.i}} \rangle\;\;\tab{1}\pcrop$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\emptyfunc}\rangle$
\end{tabular}


==> graph1_norm/tables_inc/leaf00_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{1.i}}, \tuplecolor{\statePredColor}{\sigma_{1.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{1.i}} \rangle\qquad\tab{1}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
%$\tuplecolor{\outputPredColor}{\langle\{a_1,f\}, \{r_{cf}\}\rangle, \langle\{a_2, f\}, \{r_{cf}\}\rangle,}$\\%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
%$\;\tuplecolor{\outputPredColor}{\langle\{f\}, \{r_{cf}\}\rangle, \langle\{a_1,a_2\}, \{r_c\}\rangle, }$\\%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
%$\;\tuplecolor{\outputPredColor}{\langle\{a_1\}, \{r_c\}\rangle, \langle\{a_2\}, \{r_c\}\rangle, \langle\emptyset, \{r_c\}\rangle}$\\%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
%$\;\tuplecolor{\outputPredColor}{\langle\{a_1\}, \{r_c\}\rangle, }$%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
%$\;\tuplecolor{\outputPredColor}{\langle\emptyset, \{r_1\}\rangle\}}\rangle\pcrop$\\\hline
%$\quad\tuplecolor{\outputPredColor}{\langle\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\}\rangle,}$\\
%$\quad\tuplecolor{\outputPredColor}{\langle\emptyset, \{r_1\mapstos\infty, r_2\mapstos1\}\rangle\}}\rangle\pcrop$\\\hline
%
%$\;\tuplecolor{\outputPredColor}{\langle\{a\},\{r_1\}\rangle\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\emptyset}\rangle\pcrop$%\\
%$\tuplecolor{\outputPredColor}{\langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph1_norm/tables_inc/leaf0_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{4.i}}, \tuplecolor{\statePredColor}{\sigma_{4.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{4.i}} \rangle\quad\tab{4}\pcrop$}\\
\hline\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{c\}}, \tuplecolor{\statePredColor}{\{r_1\mapstos0,r_2\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\{}$\\
$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\})\}}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty,r_2\mapstos0\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$
\end{tabular}


==> graph1_norm/tables_inc/leaf1.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{32.i}}, \tuplecolor{\statePredColor}{\sigma_{32.i}} \rangle\pcrop$}\\ % & \multicolumn{2}{c}{$M_i$}\\
%& $a$ & $d$ \\
\hline\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_c\}}, \tuplecolor{\statePredColor}{\{r_{c2}\}}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_{c2}\}}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\emptyset}\rangle\pcrop$\\
\end{tabular}


==> graph1_norm/tables_inc/leaf1_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{32.i}}, \tuplecolor{\statePredColor}{\sigma_{32.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{32.i}} \rangle\pcrop$}\\
\hline\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_c\}}, \tuplecolor{\statePredColor}{\{r_{c2}\}}, \tuplecolor{\outputPredColor}{\{}\pcrop$\\
% \{r_{c2}\}\rangle, }\pcrop$\\% \hline
$\tuplecolor{\outputPredColor}{\langle \{a_c\}, \{r_{c2}\}\rangle, }\pcrop$\\
$\tuplecolor{\outputPredColor}{ \langle\emptyset, \{r_{c2}\}\rangle\}}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_c\}}, \tuplecolor{\statePredColor}{\{r_{c2}\}}, \tuplecolor{\outputPredColor}{\{}\pcrop$\\
$\tuplecolor{\outputPredColor}{\langle \emptyset, \{r_{c2}\}\rangle\}}\rangle\pcrop$\\\hline
%$\;\tuplecolor{\outputPredColor}{(\{d\}, \emptyfunc)\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset},  \tuplecolor{\statePredColor}{\{r_{c2}\}}, \tuplecolor{\outputPredColor}{\{} \pcrop$\\
$\tuplecolor{\outputPredColor}{\langle \emptyset, \{r_{c2}\}\rangle\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset},  \tuplecolor{\statePredColor}{\{r_{c2}\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset},  \tuplecolor{\statePredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\{\langle \emptyset, \{r_{c2}\}\rangle\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset},  \tuplecolor{\statePredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\%\hline
\end{tabular}


==> graph1_norm/tables_inc/r14.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{12.i}}, \tuplecolor{\statePredColor}{\sigma_{12.i}} \rangle\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{e_{bc}, a_b\}}, \tuplecolor{\statePredColor}{\emptyset} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{e_{bc}\}}, \tuplecolor{\statePredColor}{\{r_{c1}\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_b\}}, \tuplecolor{\statePredColor}{\{r_{c1}\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_{c1}\}} \rangle\pcrop$\\%\hline
%$\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{a_1\mapstos\infty,a_2\mapstos1\}} \rangle$\\
\end{tabular}


==> graph1_norm/tables_inc/r14_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{12.i}}, \tuplecolor{\statePredColor}{\sigma_{12.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{12.i}} \rangle\,\;\;\qquad\tab{12}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{e_{bc}, a_b\}}, \tuplecolor{\statePredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\{\langle\{e_{bc}\},\{r_{c1}\}\rangle\}}\rangle\pcrop$\\\hline%\rangle$\\\hline
%$\;\tuplecolor{\outputPredColor}{\langle\{a_b\}, \{r_{c1}\}\rangle, \langle \emptyset, \{r_{c1}\}\rangle\}}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{e_{bc}, a_b\}}, \tuplecolor{\statePredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\emptyset}\rangle$\\\hline %\{\langle\{a_b\},\{r_{c1}\}\rangle\}}\rangle\pcrop$\\\hline%\rangle$\\\hline
%
$\pcrop\langle \tuplecolor{\inputPredColor}{\{e_{bc}\}}, \tuplecolor{\statePredColor}{\{r_{c1}\}}, \tuplecolor{\outputPredColor}{\emptyset}\rangle$\\\hline%\{\langle\emptyset,\{r_{c1}\}\rangle\}}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_b\}}, \tuplecolor{\statePredColor}{\{r_{c1}\}}, \tuplecolor{\outputPredColor}{\{\langle \emptyset, \{r_{c1}\} \rangle\}}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_b\}}, \tuplecolor{\statePredColor}{\{r_{c1}\}}, \tuplecolor{\outputPredColor}{\emptyset}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_{c1}\}}, \tuplecolor{\outputPredColor}{\emptyset}\rangle\pcrop$%\\\hline
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{a_1\}}, \tuplecolor{\outputPredColor}{\emptyset}\rangle$\\%\hline
%$\tuplecolor{\outputPredColor}{(\emptyset,\hspace{-0.2em}\{a_1\mapstos0\}),}\pcrop$\\
%$\quad\tuplecolor{\outputPredColor}{(\{a\}, \{a_1\mapstos\infty\})\}}\rangle$\\\hline
%
%$\pcrop\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\statePredColor}{\{a_1\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\{}$\\
%$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{a_1\mapstos0\}),}$%\\
%$\tuplecolor{\outputPredColor}{(\emptyset, \{a_1\mapstos1\}),}\pcrop$\\
%$\quad\tuplecolor{\outputPredColor}{(\{a\}, \{a_1\mapstos\infty\}),}$\\
%$\quad\tuplecolor{\outputPredColor}{(\{a\}, \{a_1\mapstos1\})\}}\rangle$\\\hline
%
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{a_1\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\emptyset}\rangle$\\\hline
%
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{a_1\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{(\emptyset, \{a_1\mapstos1\})\}}\rangle\pcrop$\\
\end{tabular}


==> graph1_norm/tables_inc/r5.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{3.i}}, \tuplecolor{\statePredColor}{\sigma_{3.i}} \rangle \;\tab{3}\pcrop$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{e_{ab}\}}, \tuplecolor{\statePredColor}{\{r_{ab}\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_{ab}\}} \rangle\pcrop$%\\\hline
%$\pcrop\langle \tuplecolor{\inputPredColor}{\{c\}}, \tuplecolor{\statePredColor}{\{r_2\}} \rangle\pcrop$\\\hline
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}\rangle$\\
\end{tabular}


==> graph1_norm/tables_inc/r5_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{3.i}}, \tuplecolor{\statePredColor}{\sigma_{3.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{3.i}} \rangle\quad\;\tab{3}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$3$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{e_{ab}\}}, \tuplecolor{\statePredColor}{\{r_{ab}\}}, \tuplecolor{\outputPredColor}{\{\langle \emptyset, \emptyset \rangle\}}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_{ab}\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph1_norm/tables_inc/r5_asp_2mdp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{3.i}}, \tuplecolor{\statePredColor}{\sigma_{3.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{3.i}} \rangle\quad\qquad\;\tab{3}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$3$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,a_2,f\}}, \tuplecolor{\statePredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\emptyset}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_2,f\}}, \tuplecolor{\statePredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph1_norm/tables_inc/r7.tex <==
\begin{tabular}{l}
\multirow{1}{*}{\pcrop$\langle \tuplecolor{\inputPredColor}{M_{7.i}}, \tuplecolor{\statePredColor}{\sigma_{7.i}} \rangle\quad\;\;\tab{7}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a,b\}}, \tuplecolor{\statePredColor}{\{r_1,r_2\}} \rangle\pcrop$ \\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a,b\}}, \tuplecolor{\statePredColor}{\{r_1\}} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1,r_2\}} \rangle$
\end{tabular}


==> graph1_norm/tables_inc/r8.tex <==
\begin{tabular}{l}
\multirow{1}{*}{\pcrop$\langle \tuplecolor{\inputPredColor}{M_{6.i}}, \tuplecolor{\statePredColor}{\sigma_{6.i}}\rangle\quad\tab{6}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{e_{ab}, a_b\}}, \tuplecolor{\statePredColor}{\{r_b\}} \rangle\pcrop$ \\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{e_{ab}\}}, \tuplecolor{\statePredColor}{\emptyset} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_b\}}, \tuplecolor{\statePredColor}{\{r_b\}} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_b\}} \rangle$
\end{tabular}


==> graph1_norm/tables_inc/r8_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{6.i}}, \tuplecolor{\statePredColor}{\sigma_{6.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{6.i}} \rangle\quad\tab{6}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{e_{ab}, a_b\}}, \tuplecolor{\statePredColor}{\{r_b\}}, \tuplecolor{\outputPredColor}{\{}$\\
$\tuplecolor{\outputPredColor}{\langle\{e_{ab}\}, \emptyset\rangle\}}\rangle\pcrop$\\\hline
%$\;\tuplecolor{\outputPredColor}{\langle\{a_b\}, \{r_b\}\rangle\}}\rangle$\\\hline%b\}, \{a_1\}), (\emptyset, \{a_1\})\}} \rangle\pcrop$\\\hline
%$\;\tuplecolor{\outputPredColor}{(\emptyset, \{a_1\})\}}\rangle\pcrop$\\\hline
%$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\}),}$\\
%$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos1\})\}}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{e_{ab}\}}, \tuplecolor{\statePredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\emptyset}\rangle\pcrop$\\\hline
%$\;\tuplecolor{\outputPredColor}{(\{a\},\{r_1\})\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_b\}}, \tuplecolor{\statePredColor}{\{r_b\}}, \tuplecolor{\outputPredColor}{\{\langle \emptyset, \{r_b\} \rangle\}} \rangle\pcrop\hspace{-0.1em}$\\\hline
%$\pcrop\langle \tuplecolor{\inputPredColor}{\{b\}}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{(\emptyset,\emptyset)\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_b\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$%\\\hline
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph1_norm/tables_inc/r8_asp_2.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{1.i}}, \tuplecolor{\statePredColor}{\sigma_{1.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{1.i}} \rangle\quad\qquad\qquad\qquad\qquad\qquad\;\tab{1}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,a_2,f\}}, \tuplecolor{\statePredColor}{\{r_c, r_{cf}\}}, \tuplecolor{\outputPredColor}{\{}\pcrop$\\
$\;\tuplecolor{\outputPredColor}{\langle\{a_1,f\}, \{r_{cf}\}\rangle, \langle\{a_2, f\}, \{r_{cf}\}\rangle,}$\\%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
$\;\tuplecolor{\outputPredColor}{\langle\{f\}, \{r_{cf}\}\rangle, \langle\{a_1,a_2\}, \{r_c\}\rangle, }$\\%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
$\;\tuplecolor{\outputPredColor}{\langle\{a_1\}, \{r_c\}\rangle, \langle\{a_2\}, \{r_c\}\rangle, \langle\emptyset, \{r_c\}\rangle\}}\rangle$\\\hline%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
%$\;\tuplecolor{\outputPredColor}{}\rangle$\\%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
%$\;\tuplecolor{\outputPredColor}{\langle\emptyset, \{r_1\}\rangle\}}\rangle\pcrop$\\\hline
%$\quad\tuplecolor{\outputPredColor}{\langle\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\}\rangle,}$\\
%$\quad\tuplecolor{\outputPredColor}{\langle\emptyset, \{r_1\mapstos\infty, r_2\mapstos1\}\rangle\}}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,a_2\}}, \tuplecolor{\statePredColor}{\{r_c, r_{cf}\}}, \tuplecolor{\outputPredColor}{}\pcrop$\\
$\;\tuplecolor{\outputPredColor}{\langle\{a_1\}, \{r_c, r_{cf}\}\rangle, \langle\{a_2\}, \{r_c, r_{cf}\}\rangle,}$\\%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
$\;\tuplecolor{\outputPredColor}{\langle\emptyset, \{r_c, r_{cf}\}\rangle\}}\rangle$\\\hline%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
%
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,f\}}, \tuplecolor{\statePredColor}{\{r_c, r_{cf}\}}, \tuplecolor{\outputPredColor}{\{\langle\{f\}, \{r_{cf}\}\rangle,}\pcrop$\\
$\;\tuplecolor{\outputPredColor}{\langle\{a_1\}, \{r_{c}\}\rangle, \langle\emptyset, \{r_c\}\}\rangle\}}\rangle$\\\hline%b\}, \{r_1\}\rangle, \langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1\}}, \tuplecolor{\statePredColor}{\{r_c, r_{cf}\}}, \tuplecolor{\outputPredColor}{\{\langle\emptyset, \{r_c, r_f\}\rangle\}}\rangle$\\\hline
%$\;\tuplecolor{\outputPredColor}{\langle\{a\},\{r_1\}\rangle\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_2,f\}}, \tuplecolor{\statePredColor}{\{r_c,r_{cf}\}}, \tuplecolor{\outputPredColor}{\{\langle\{a_2\}, \{r_c\}\rangle, \langle\{f\}, \{r_{cf}\}\rangle \}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_2\}}, \tuplecolor{\statePredColor}{\{r_c, r_{cf}\}}, \tuplecolor{\outputPredColor}{\{\langle\emptyset,\{r_c, r_{cf}\}\rangle\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{f\}}, \tuplecolor{\statePredColor}{\{r_c, r_{cf}\}}, \tuplecolor{\outputPredColor}{\{\langle\emptyset, \{r_c\}\rangle\}} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_c, r_{cf}\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{\langle\emptyset, \{r_1\}\rangle\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph1_norm/tables_inc/r8_asp_2mdp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{1.i}}, \tuplecolor{\statePredColor}{\sigma_{1.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{1.i}} \rangle\quad\qquad\;\tab{1}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,a_2,f\}}, \tuplecolor{\statePredColor}{\{r_c, r_{cf}\}}, \tuplecolor{\outputPredColor}{\emptyset}\pcrop$\\
%$\;\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}}\rangle\pcrop$\\\hline
%$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\}),}$\\
%$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos1\})\}}\rangle\pcrop$\\\hline
%
%$\;\tuplecolor{\outputPredColor}{(\{a\},\{r_1\})\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_2,f\}}, \tuplecolor{\statePredColor}{\{r_c,r_{cf}\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph1_norm/tables_inc/r8_asp_2mdp_tmp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{1.i}}, \tuplecolor{\statePredColor}{\sigma_{1.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{1.i}} \rangle\quad\qquad\;\tab{1}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,a_2,f\}}, \tuplecolor{\statePredColor}{\{r_c, r_{cf}\}}, \tuplecolor{\outputPredColor}{}\pcrop$\\
$\;\tuplecolor{\outputPredColor}{(\{a_1,f\}, \{r_{cf}\}), (\{a_2, f\}, \{r_{cf}\}),}$\\%b\}, \{r_1\}), (\emptyset, \{r_1\})\}} \rangle\pcrop$\\\hline
$\;\tuplecolor{\outputPredColor}{(\{f\}, \{r_{cf}\}),}$\\%b\}, \{r_1\}), (\emptyset, \{r_1\})\}} \rangle\pcrop$\\\hline
$\;\tuplecolor{\outputPredColor}{(\{a_1,a_2\}, \{r_c\}), (\{a_1\}, \{r_c\})\}}\rangle$\\%b\}, \{r_1\}), (\emptyset, \{r_1\})\}} \rangle\pcrop$\\\hline
$\;\tuplecolor{\outputPredColor}{(\{a_2\}, \{r_c\}), (\{a_1\}, \{r_c\}), (\emptyset, \{r_c\})\}}\rangle$\\\hline%b\}, \{r_1\}), (\emptyset, \{r_1\})\}} \rangle\pcrop$\\\hline
%$\;\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}}\rangle\pcrop$\\\hline
%$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\}),}$\\
%$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos1\})\}}\rangle\pcrop$\\\hline
%
%$\;\tuplecolor{\outputPredColor}{(\{a\},\{r_1\})\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_2,f\}}, \tuplecolor{\statePredColor}{\{r_c,r_{cf}\}}, \tuplecolor{\outputPredColor}{\{(\{a_2\}, \{r_c\}), (\{f\}, \{r_{cf}\}) \}} \rangle$\\
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph1_norm/tables_inc/r9_asp_2.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{2.i}}, \tuplecolor{\statePredColor}{\sigma_{2.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{2.i}} \rangle\quad\qquad\;\tab{2}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,a_2,f\}}, \tuplecolor{\statePredColor}{\{r_f, r_2\}}, \tuplecolor{\outputPredColor}{\emptyset}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,a_2\}}, \tuplecolor{\statePredColor}{\{r_2\}}, \tuplecolor{\outputPredColor}{\{\langle\{a_1\}, \emptyset\rangle}\pcrop$\\
$\;\tuplecolor{\outputPredColor}{\langle\{a_2\}, \{r_2\}\rangle, \langle\emptyset, \emptyset\rangle\}}\rangle$\\\hline%b\}, \{r_1\}), (\emptyset, \{r_1\})\}} \rangle\pcrop$\\\hline
%
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,f\}}, \tuplecolor{\statePredColor}{\{r_{f}\}}, \tuplecolor{\outputPredColor}{\emptyset}\rangle$\\\hline
%$\;\tuplecolor{\outputPredColor}{\emptyset}\rangle$\\\hline%b\}, \{r_1\}), (\emptyset, \{r_1\})\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1\}}, \tuplecolor{\statePredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\{\langle\emptyset, \emptyset\rangle\}}\rangle$\\\hline
%$\;\tuplecolor{\outputPredColor}{(\{a\},\{r_1\})\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_2,f\}}, \tuplecolor{\statePredColor}{\{r_{f}, r_2\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_2\}}, \tuplecolor{\statePredColor}{\{r_2\}}, \tuplecolor{\outputPredColor}{\{\langle\emptyset,\emptyset\rangle\}}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{f\}}, \tuplecolor{\statePredColor}{\{r_f\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$%\\\hline
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph1_norm/tables_inc/r9_asp_2mdp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{2.i}}, \tuplecolor{\statePredColor}{\sigma_{2.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{2.i}} \rangle\quad\qquad\;\tab{2}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_1,a_2,f\}}, \tuplecolor{\statePredColor}{\{r_f, r_2\}}, \tuplecolor{\outputPredColor}{\emptyset}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a_2,f\}}, \tuplecolor{\statePredColor}{\{r_{f}, r_2\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\
%$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\}}, \tuplecolor{\outputPredColor}{\{}$%\\
%$\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\})\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> prim.tex <==
%
% NEW VERSION 
%
%\vspace{-5ex}
 \begin{algorithm}[t]
   %\KwData{Program $\prog$, Node $t$, childtables~$\tab{t'}$ and $\tab{t''}$ (if exist(s)), of fixed TD~$\TTT$ of $P(\prog)$.}%
   \KwData{Bag $\chi_t$, bag-rules $\prog_t$ and child tables $\Tab{}$ of node $t$.{~\bf Out:} Table~$\tab{t}$.} % of fixed TD~$\TTT$ of $P(\prog)$, and tables~$\tab{t'}, \dots, \tab{t''}$ of child nodes of $t$.}%
   %\KwData{Bag-atoms $A_t$, bag-rules $\prog_t$ and child tables $\Tab{}$ of node $t$.{~\bf Out:} Table~$\tab{t}$.} % of fixed TD~$\TTT$ of $P(\prog)$, and tables~$\tab{t'}, \dots, \tab{t''}$ of child nodes of $t$.}%
   %\KwData{Corresponding atoms $A_t$, rules $\prog_t$ and child tables $\Tab{}$ of node $t$.} % of fixed TD~$\TTT$ of $P(\prog)$, and tables~$\tab{t'}, \dots, \tab{t''}$ of child nodes of $t$.}%
   %\KwResult{Table~$\tab{t}$ for node $t$.}%
   %
   %$\prog_t^M\eqdef (\prog_t)^M$\;
   %({R}_t)^M \SE$\;%
   %$\Mod(\CCC,\prog) \eqdef \SB C \SM C \in \CCC, C \models \prog \SE$\;
   %$\CCC \sqcup \{a\} \eqdef \SB C \cup \{a\} \SM C \in \CCC \SE$\;
   \lIf(\tcc*[f]{Abbreviations see
     Footnote~\ref{foot:abrev}.}){$\type(t) = \leaf$}{%
     $\tab{t} \eqdef \Big\{ \Big\langle
     \tuplecolor{\inputPredColor}{\emptyset},~\tuplecolor{\outputPredColor}{\emptyset}
     \Big\rangle \Big\}$%
     % 
 	%\EndIIf 
   }%
  \uElseIf{$\type(t) = \intr$, $a\in \chi_t$ is introduced and $\tau'\in \Tab{}$}{
   \vspace{-0.25em}
   \makebox[7.39cm][l]{$\tab{t} \eqdef \Big\{ \Big\langle \tuplecolor{\inputPredColor}{\MAI{M}},~\tuplecolor{\outputPredColor}{\Mod(\{M\} \cup [\CCC \sqcup \{ a \}] \cup \CCC, \prog_t^{\MAI{M}
     })} \Big\rangle$}%\;\cup\; \Mod(\CCC \sqcup \{ a \}, \prog_t^{(M \cup \{a\})})%
     %\;\cup\; \Mod_t(\{M\},M \cup \{a\}) \Big\rangle$\\
     $\Bigm|\;\langle \tuplecolor{\inputPredColor}{M}, \tuplecolor{\outputPredColor}{\CCC} \rangle \in \tab{}',  \tuplecolor{\inputPredColor}{\MAI{M}}
     \models {\prog}_t \Big\} \;\mcup$
   
   %\Big\{ \Big\langle M, \Mod(\CCC,\prog_t^M)\Big\rangle$}%
   %$\Bigm| \langle M, \CCC
   %\rangle \in \tab{t'}, M \models {R}_t \Big\} \;\mcup$\\
     %
     \makebox[7.39cm][l]{\qquad$\,\,\,\hspace{0.07em}\Big\{ \Big\langle \tuplecolor{\inputPredColor}{M},~ \tuplecolor{\outputPredColor}{\Mod(\CCC,\prog_t^M)}\Big\rangle$}%
   $\Bigm|\;\langle \tuplecolor{\inputPredColor}{M}, \tuplecolor{\outputPredColor}{\CCC}
   \rangle \in \tab{}', \tuplecolor{\inputPredColor}{M} \models {\prog}_t \Big\}$
   \vspace{-0.05em}
     %\Big\{ \Big\langle \MAI{M}, \Mod(\CCC \cup [\CCC \sqcup \{ a \}] \cup \{M\}, \prog_t^{\MAI{M}
     %}) \Big\rangle$}%\;\cup\; \Mod(\CCC \sqcup \{ a \}, \prog_t^{(M \cup \{a\})})%
     %%\;\cup\; \Mod_t(\{M\},M \cup \{a\}) \Big\rangle$\\
     %$\Bigm| \langle M, \CCC \rangle \in \tab{t'},  \MAI{M}
     %\models {R}_t \Big\}$
       % 
     }\vspace{-0.05em}%
     \uElseIf{$\type(t) = \rem$, $a \not\in \chi_t$ is removed and $\tau'\in \Tab{}$}{%} and let $a \in  A_{t'} \setminus A_t$}{%
       \makebox[7.39cm][l]{$\tab{t} \eqdef \Big\{ \Big\langle \tuplecolor{\inputPredColor}{\MAR{M}},~\tuplecolor{\outputPredColor}{\{ \MAR{C}
       \mid C \in \CCC \}}\Big\rangle$}$\Bigm|\;\langle \tuplecolor{\inputPredColor}{M}, \tuplecolor{\outputPredColor}{\CCC}
       \rangle \in \tab{}' \Big\}$
   \vspace{-0.3em}
     %
     } %
     \uElseIf{$\type(t) = \join$ and $\tau', \tau'' \in \Tab{}$ with $\tau' \neq \tau''$}{%
       \makebox[7.39cm][l]{$\tab{t} \eqdef \Big\{ \Big\langle \tuplecolor{\inputPredColor}{M},~ \tuplecolor{\outputPredColor}{(\CCC' \cap \CCC'') \cup (\CCC' \cap \{M\}) \cup (\{M\}
       \cap \CCC'')}\Big\rangle$}$\Bigm|\;\langle \tuplecolor{\inputPredColor}{M}, \tuplecolor{\outputPredColor}{\CCC'}
       \rangle \in \tab{}', \langle \tuplecolor{\inputPredColor}{M}, \tuplecolor{\outputPredColor}{\CCC''} \rangle \in \tab{}''
       \Big\}$
       %
   \vspace{-0.15em}
     } 
     \vspace{-0.15em}
     %\Return $\tab{t}$\;
   %\medskip
 \caption{Table algorithm~$\algo{PRIM}(t,\chi_t,\prog_t,\cdot,\Tab{})$ 1pass. TODO: extension pointers}
   %\vspace{-2ex}
   \label{fig:prim}
 \end{algorithm}%
%\vspace{-5ex}
%\normalsize
%\vspace{-0.4cm}
%\caption{\textsf{PRIM} Algorithm.}
%\end{subfigure}%
%\normalsize
%\vspace{-0.4cm}
%\caption{\textsf{PRIM} Algorithm and extension \textsf{PRIM+C} handling model costs.}
%\label{fig:prims}
%\end{figure}
%
%OLD version
%\begin{figure}
%\small
%\noindent {\large\makebox[2.3cm][l]{\bf{Input}} {\bf Node $t$} and
%  {\bf{tables $\tab{t'}$}} and {\bf{$\tab{t''}$}} of children~$t'$ and
%  $t''$, if exist, of $t$, and\\
%  \mbox{~~~}\qquad\qquad$a \in A_t \setminus A_{t'}$ and
%  $a \in A_{t'} \setminus A_{t}$, respectively.}
%
%\smallskip {\large\makebox[2.3cm][l]{\bf{Output}} {\bf{Tuple set
%      $\tab{t}$}} of node $t$}
%
%\medskip
%\medskip
%%$\mathop{LEAF:} \Big\{ \Big\langle \emptyset, \emptyset \Big\rangle \Big\}$
%\makebox[2.3cm][l]{$t\in
%  \LEAF(\TTT)$}$\Big\{ \Big\langle \emptyset, \emptyset \Big\rangle \Big\}$
%
%\medskip
%
%\makebox[2.3cm][l]{$t\in
%  \AI(\TTT)$}\makebox[8.3cm][l]{$\Big\{ \Big\langle M,~\{ A \mid A \in
%  C, \forall r \in \hat{R}_t: A \models r^M \}\Big\rangle$}
%$\Bigm| \langle M, C \rangle \in \tab{t'}, \forall r \in \hat{R}_t: M
%\models r \Big\} \;\mcup$
%
%\medskip
%
%\makebox[2.3cm][l]{\quad\qquad\;\,}$\Big\{ \Big\langle M,~$
%$\{ A \mid A \in C, \forall r \in \hat{R}_t: A \models r^M \} \;\cup$
%
%~~~\quad\qquad\qquad\qquad\;\;$\{ A \cup \{ a \} \mid A \in C, \forall r \in
%\hat{R}_t: A \cup \{ a \} \models
%r^M \} \;\cup$
%
%%\smallskip
%~~~\quad\qquad\qquad\qquad\;\;$\{ M'' | M'' = M', \forall r \in \hat{R}_t: M''
%\models r^M \}\Big\rangle$
%
%\makebox[8.3cm][l]{\hfill\qquad\qquad}$ \Bigm| \langle M', C \rangle \in \tab{t'}, M = M'
%\cup \{ a \}, \forall r \in \hat{R}_t: M \models r \Big\}$
%
%\medskip
%\medskip
%
%\makebox[2.3cm][l]{$t\in
%  \AR(\TTT)$}\makebox[8.3cm][l]{$\Big\{ \Big\langle M \setminus \{ a \}, \{ A \setminus \{ a \}
%\mid A \in C \}\Big\rangle$}
%$\Bigm| \langle M, C \rangle \in \tab{t'}
%\Big\}$
%
%\medskip
%\medskip
%\makebox[2.3cm][l]{$t\in
%  \JOIN(\TTT)$}\makebox[8.3cm][l]{$\Big\{ \Big\langle  M,~(C' \cap C'') \cup (\{M\} \cap
%C'') \cup (C' \cap \{M\})\Big\rangle$}
%$\Bigm| \langle M, C' \rangle \in \tab{t'}, \langle M, C''
%\rangle \in \tab{t''} \Big\}$
%
%
%% \begin{eqnarray*}
%%   AI(a): & \{ \langle & M,\\
%%   %
%%   && \{ A \mid A \in C, \forall r \in {R}_t: A \models r^M \}\rangle,\\
%%   %
%%   & \mid & \langle M, C \rangle \in \tab{t'}, \forall r \in {R}_t: M
%%   \models r\} \cup\\
%%   %
%%   & \{ \langle & M,\\
%%   %
%%   && \{ A \mid A \in C, \forall r \in {R}_t: A \models r^M \} \cup\\
%%   %
%%   && \{ A \cup \{ a \} \mid A \in C, \forall r \in {R}_t: A \cup \{ a \} \models
%%   r^M \} \cup\\
%%   %
%%   && \{ M'' \mid M'' = M', \forall r \in {R}_t: M'' \models r^M \}\rangle\\
%%   %
%%   & \mid & \langle M', C \rangle \in \tab{t'}, M = M' \cup \{ a \} \}\\
%%   %
%%   \\[-2ex]
%%   %
%%   AR(a): & \{ \langle & M \setminus \{ a \}, \{ A \setminus \{ a \} \mid A \in C
%%   \}\rangle\\
%%   %
%%   & \mid & \langle M, C \rangle \in \tab{t'} \}\\
%%   %
%%   \\[-2ex]
%%   %
%%   JOIN: & \{ \langle & M, (C' \cap C'') \cup (\{M\} \cap C'') \cup (C' \cap \{M\})\rangle\\
%%   %
%%   & \mid & \langle M, C' \rangle \in \tab{t'}, \langle M, C'' \rangle \in
%%   \tab{t''} \}\\
%%   %
%%   \\[-2ex]
%%   %
%%   LEAF: && \{ \langle \emptyset, \emptyset \rangle \}
%% \end{eqnarray*}
%\caption{The algorithm~\algo{PRIM}.}
%\vspace{-2ex}
%\label{fig:prim}
%\end{figure}
%
%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: epia2017"
%%% End:

